Equivariant dendroidal sets and simplicial operads

We establish a Quillen equivalence between the homotopy theories of equivariant Segal operads and equivariant simplicial operads with norm maps. Together with previous work, we further conclude that the homotopy coherent nerve is a right-Quillen equivalence from the model category of equivariant simplicial operads with norm maps to the model category structure for equivariant-$\infty$-operads in equivariant dendroidal sets.

==> labels-TAS.tex <==
% Rigidification Aux File


% OneColor Aux File



% AllColors-v2 aux file


